On Gradient Coding with Partial Recovery

We consider a generalization of the gradient coding framework where a dataset is divided across $n$ workers and each worker transmits to a master node one or more linear combinations of the gradients over its assigned data subsets. Unlike the conventional framework which requires the master node to recover the sum of the gradients over all the data subsets in the presence of straggler workers, we relax the goal to computing the sum of at least some $\alpha$ fraction of the gradients. We begin by deriving a lower bound on the computation load of any scheme and also propose two strategies which achieve this lower bound, albeit at the cost of high communication load and a number of data partitions which can be polynomial in $n$. We then propose schemes based on cyclic assignment which utilize $n$ data partitions and have a lower communication load. When each worker transmits a single linear combination, we prove lower bounds on the computation load of any scheme using $n$ data partitions. Finally, we describe a class of schemes which achieve different intermediate operating points for the computation and communication load and provide simulation results to demonstrate the empirical performance of our schemes.

==> Additional_Notes.tex <==
$|\bigcup\limits_{j \in S} E_j|=|B|(1-\frac{{v-t \choose p}}{{v \choose p}})$ for every $S$ satisfying $|S|=n-s$.

Note that since the given assignment is a $t$-design, $|\bigcap\limits_{j \in S} E_j|=\lambda$. Also using the inclusion-exclusion principle for sets, we know that 

$$|\bigcup_{i\in [m]} C_i|= \sum_{i \in [m]} |C_i| - \sum_{1\leq i< j\leq m}|C_i\cap C_j|+\sum_{1\leq i< j<k\leq m}|C_i\cap C_j\cap C_k| + ..+(-1)^m|C_1\cap C_2\cap \ldots \cap C_m| $$

Note that in this case $C_i$ denote the set $E_i$ and $[m]$ denotes an possible subset $S$ with $|S|=n-s=t$. Now we know that $|C_1\cap C_2\cap \ldots \cap C_m|=\lambda$ and similarly $|C_{i_1}\cap C_{i_2} \cap \ldots \cap C_{i_a}|= \lambda \prod_{i=1}^{a} \frac{(v - t + i)}{(p - t + i)}$. Also, $\lambda=|B|\frac{{p \choose t}}{{v \choose t}}$ which can be shown on repeated application of the above result. 

Thus, the above expression evaluates to $|B|(\sum_{i=1}^{t} (-1)^i \frac{{p \choose i}}{{v \choose i}}. {{t \choose i}})= \frac{|B|}{{v \choose p}}(\sum_{i=1}^{t} (-1)^{i-1} {{v-i\choose v-p}}.{{t \choose i}})=|B|(1-\frac{{v-t \choose p}}{{v \choose p}})$. 


\remove{Note that, the above expression can be computed using the idea of binomial expressions. Note that ${{k \choose i}}$ denotes the coefficient of $x^{i}$ in $(1+x)^k$ and $(-1)^i\times {{v-i\choose v-k}}$ denotes coefficient of $x^{(p-i)}$ in $(1+x)^{-(v-p+1)}$. Thus the numerator of the above expression is ${{v \choose p}}$ plus the coefficient of $x^p$ in $-(1+x)^t\times (1+x)^{-(v-p+1)}=-(1+x)^{-(v-p-t+1)}$ thus equals ${{v \choose p}}-{{v-t \choose p}}$. Hence, proved.}



%Thus, combining the fact that every $t$-design is a $u$-design for every $u \leq t$, we can show that $|\bigcup\limits_{j \in S} E_j|$ is fixed for every $S$ satisfying $|S|=n-s$

\remove{
\begin{lemma}
$|\bigcup\limits_{j \in S} E_j|={{v-t \choose k}}$ for every $|S|=t$
\end{lemma}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now derive a scheme based on the scheme proposed in Theorem \ref{high_comm_cyclic_middle_thm} which incurs a lower communication cost under the same computation load for a subset of parameters. {\color{red} Note that the inequality \eqref{high_comm_cyclic_middle_eqn2} is same as \eqref{high_comm_cyclic_middle_eqn1}.}

\remove{We now compute the number of data-partitions assigned to any of $n-s$ continuous workers whose indices are denoted by $I$.\remove{ We denote $J_i= \cup_{t \in I} {j:0\leq (t-j \mod n) \leq \gamma_i}$ for every $i \in [y]$ which denotes set of all possibilities for $i^{th}$ element in the list corresponding to the spanned data-partitions.} W.L.O.G, we assume that the indices of the non-straggled workers are $1,2,\ldots, n-s$. Consider all data-partitions not assigned to any of these workers whose $i^{th}$ element in the corresponding list is the largest, suppose we denote such a list by $\{c_1,c_2,\ldots c_y\}$. Thus, $c_i \leq (n-\gamma_i+1)$, $(c_{(j \mod n)+1)}-c_j) \geq \gamma_j$ for $j \in [y]$ and $c_{i+1}\geq n-s+1$. Thus, the number of such lists with the largest element being the $i^{th}$ element is given by ${{s-(\gamma_i)-\sum_{i=1}^{y-1}\gamma_i+y \choose y}}={{s-\delta+y \choose y}}$ as $\delta= \sum_{i=1}^{y}\gamma_i$. Thus, the total number of data-partitions not assigned to any of the consecutive $n-s$ workers is given by $y.{{s-\delta+y \choose y}}$. Thus, the number of gradients received at the master when consecutive $s$ workers straggle is given by $n.{{n-\delta+y-1 \choose y-1}}-y.{{s-\delta+y \choose y}}$.

\noindent {\bf Step 4: Lower bound on the number of data-partitions assigned to non-consecutive workers:} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\remove{
Note that for the case of $\gamma=1$, this parameter of this scheme is same as that of the scheme described in Sec ~\ref{compload_ub_section} where as for the case of $y=1$ it become same as that of the cyclic schemes as in Sec ~\ref{cyclic_scheme_section} except with a bit higher communication cost of $\gamma$ (transmitting all the data-partitions assigned). We denote $\gamma^{*}(y)$ as the minimum value of $\gamma$ satisfying the inequality \eqref{high_comm_cyclic_middle} for a given value of $y$. We can show that the computation load $\gamma^{*}(y).y$ typically decreases from the cyclic computation load in Sec ~\ref{cyclic_scheme_section} to Sec ~\ref{compload_ub_section} to as $y$ increases from 1 (stated as a corollary below) and the communication cost (as a function of $\gamma^{*}$ and $y$) decreases as $y$ increases from 1.

Thus, these give another set of gradient codes with computation load between the cyclic codes as discussed in Sec ~\ref{cyclic_scheme_section} and the optimal computation load as attained in Sec ~\ref{compload_ub_section}. Also note that the communication cost in this scheme typically lies between the two extremes.
}


Recall the assignment of data-partitions to workers described in the proof of Theorem~\ref{high_comm_cyclic_middle} where each data-partition is denoted by a list of size $y$ with integers $\{\gamma_i\}_{i=1}^{y}$ chosen satisfying $\sum_i{\gamma_i}=\delta$. We impose the additional constraint that $(c_{1+(i \mod n)}-c_i \mod n) \geq \gamma_i$ $\forall i \in [y]$. Note that corresponding to each such unique list, we had a unique data-partition. Now a data-partition denoted by the list ($[c_1,c_2,\ldots,c_y]$) is assigned to worker $W_j$ iff $0 \leq ((j - c_i) \mod n) \leq \gamma_i-1$ for some $i \in [y]$.



However, for the case of $\delta=y$ the communication cost of this scheme is $y$ times that of the one in Section ~\ref{compload_ub_section} whereas for the case of $y=1$, the communication cost is $\delta$(transmitting gradients of all the data-partitions assigned) unlike the scheme in Section ~\ref{cyclic_scheme_section} with communication cost of 1 or 2.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[ht]
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[scale =0.5]{comp_load_v2_n_20_s_7_alpha_998.png}
\caption{Computation load with $y$ for $n=20$, $s=7$, $\alpha=0.998$}
\label{comp_load_n_20_s_7_alpha_998}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[scale = 0.5]{comm_load_v2_n_20_s_7_alpha_998.png}
\caption{Communication cost with $y$ for $n=20$, $s=7$, $\alpha=0.998$}
\label{comm_cost_n_20_s_7_alpha_998}
\end{minipage}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[ht]
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[scale =0.5]{comp_load_v2_n_19_s_10_alpha_9998.png}
\caption{Computation load with $y$ for $n=19$, $s=10$, $\alpha=0.9998$}
\label{comp_load_n_19_s_10_alpha_9998}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[scale = 0.5]{comm_load_v2_n_19_s_10_alpha_9998.png}
\caption{Communication cost with $y$ for $n=19$, $s=10$, $\alpha=0.9998$}
\label{comm_cost_n_19_s_10_alpha_9998}
\end{minipage}
\end{figure}

Note that the values of $\delta^{*}(y)$ takes values $[11, 11, 11, 11, 11, 10, 10, 9, 9]$ for $y = [1,2,3,4,5,6,7,8,9]$ in Fig ~\ref{comp_load_n_19_s_10_alpha_9998},\ref{comm_cost_n_19_s_10_alpha_9998}. We plot the communication and computation cost according to Corollary ~\ref{high_comm_cyclic_middle_corollary}.




==> proof_cyclic_constr_2_short.tex <==
\section{Correctness argument of the construction proposed in Theorem \ref{cyclic_constr_comm_2}}\label{cyclic_constr_comm_2_proof}


The proof follows by going through the Algorithm \ref{back_move_straggler} and arguing along similar lines as in the proof of Theorem \ref{cyclic_constr_comm_1}. The key difference as compared to the proof of Theorem \ref{cyclic_constr_comm_1} is that in this case we have to recover sum of $\beta+x$ gradients, where $x=\beta \mod (s+1+\beta-n)$. Hence, in addition to picking the non straggling workers from the groups, we need to pick another non straggling worker which additionally gives sum of $x$ gradients. The details of the proof are given in \cite{sarmasarkar2021gradient}.


==> proof_interim_points_backup.tex <==
\section{Proof of Theorem \ref{high_comm_cyclic_middle_thm}}{\label{high_comm_cyclic_section}}

We now compute the number of data-partitions assigned to any of $n-s$ continuous workers whose indices are denoted by $I$.\remove{ We denote $J_i= \cup_{t \in I} {j:0\leq (t-j \mod n) \leq \gamma_i}$ for every $i \in [y]$ which denotes set of all possibilities for $i^{th}$ element in the list corresponding to the spanned data-partitions.} W.L.O.G, we assume that the indices of the non-straggled workers are $1,2,\ldots, n-s$. Consider all data-partitions not assigned to any of these workers whose $i^{th}$ element in the corresponding list is the largest, suppose we denote such a list by $\{c_1,c_2,\ldots c_y\}$. Thus, $c_i \leq (n-\gamma_i+1)$, $(c_{(j \mod n)+1)}-c_j) \geq \gamma_j$ for $j \in [y]$ and $c_{i+1}\geq n-s+1$. Thus, the number of such lists with the largest element being the $i^{th}$ element is given by ${{s-(\gamma_i)-\sum_{i=1}^{y-1}\gamma_i+y \choose y}}={{s-\delta+y \choose y}}$ as $\delta= \sum_{i=1}^{y}\gamma_i$. Thus, the total number of data-partitions not assigned to any of the consecutive $n-s$ workers is given by $y.{{s-\delta+y \choose y}}$. Thus, the number of gradients received at the master when consecutive $s$ workers straggle is given by $n.{{n-\delta+y-1 \choose y-1}}-y.{{s-\delta+y \choose y}}$.

Suppose the straggling workers are not consecutive and can be split into $(t+1)$ disjoint consecutive groups of indices. Let us denote the set of indices of straggling workers by $I_1,I_2,\ldots,I_{t+1}$ which are increasingly ordered.  W.L.O.G, we assume that that the elements in $I_1$ are numbered from $\{1,2,\ldots,z_1\}$ and the elements in $I_2$ are numbered from $\{z_2,\ldots,z_3\}$ and so on till $\{z_{2(t-1)},\ldots,z_{2t-1}\}$. Note that $1\leq z_1 <z_2 \leq z_3 < z_4 \leq z_5 ...<z_{2((t-1)}\leq z_{2t-1}$. Now consider any data-partition which is not assigned to any of the non-straggling $n-s$ workers and we consider lists corresponding to all such data-partitions such that the $i^{th}$ element in the list being the smallest. Note that all the elements in the list corresponding to the data-partition not assigned to any of the $n-s$ non-straggling workers would be contained in either $I_1,I_2,\ldots,I_{t+1}$. 

Now we construct a list denoted by $J$ of length $s$ by appending all elements in $I_1,I_2,\ldots,I_{t+1}$ in order. Now consider all the elements in this list which are the elements of the list  $K=[c_1,c_2,\ldots,c_y]$ denoting the data-partition not assigned to any of non-straggling workers which precisely contains $y$ elements. Note that the elements in the list would be ordered as $c_i<c_{i+1}<\ldots<c_y<c_1<\ldots <c_{i-1}$. 


We can argue that the indices of these elements in $J$ would also be separated by $\gamma_i,\gamma_{i+1},\ldots,\gamma_y,\gamma_1,\ldots$ and the index of the element $c_{i-1}$ in $J$ would be at most $s-\gamma_{i-1}+1$. We argue by contradiction. 


Consider any two elements $c_t$ and $c_{t+1}$ and suppose they belong in the same list $I_u$, in which case their indices in $J$ must differ by at least $\gamma_t$ to satisfy the condition that $c_{t+1}-c_t \geq \gamma_t$. Suppose they belong in two different
lists $I_u$ and $I_v$ with $v>u$, in which case there must be at least $\gamma_t-1$ elements larger than $c_t$ in list $I_u$. This is because, workers numbered $c_t,c_t+1,\ldots,c_t+\gamma_t-1$ would be assigned the data subset corresponding to list $K=[c_1,c_2,\ldots,c_y]$ each of which must be a straggling worker as this data subset is not assigned to any of the non-straggling workers. Thus, the elements from $c_t,c_t+1,\ldots,c_t+\gamma_t-1$ would be present in list $I_u$, hence there would be at least $\gamma_t-1$ elements between $c_t$ and $c_{t+1}$ as all elements of list $I_u$ have lower index in $J$ than those elements of list $I_v$ as $v>u$. Similarly, there would be at least $\gamma_{i-1}-1$ with index higher than $c_{i-1}$ in list $J$.


Thus, the indices of these elements in $J$ would also differ by $\gamma_i,\gamma_{i+1},\ldots,\gamma_y,\gamma_1,\ldots$ and the index of the element $c_{i-1}$ in $J$ would be at most $s-\gamma_{i-1}+1$. Also note that the indices of these elements in $J$ would be different for every distinct list $[c_1,c_2,\ldots,c_y]$. Thus, the number of such lists having the $i^{th}$ element as the smallest index would be bounded by ${{s-\delta+y \choose y}}$ (as the setting is similar to the case of $n-s$ consecutive non-straggling workers), thus the total number of such lists is bounded by $y.{{s-\delta+y \choose y}}$. Hence at most $y.{{s-\delta+y \choose y}}$ data subsets would not be assigned to any of $n-s$ non-straggling workers, hence this scheme would be $(\alpha,s)$ feasible for $\alpha \leq 1- \frac{y.{{s-\delta+y \choose y}}}{n.{{n-\delta+y-1 \choose y-1}}}$.

Let us now compute the number of data-partitions not assigned to one worker. Using a similar technique as used previously, we argue that $y.{{n-1-\delta+y \choose y}}$ data subsets would not be assigned to that worker, thus the communication cost incurred by this scheme is $(n.{{n-\delta+y-1 \choose y-1}}-y.{{n-1-\delta+y \choose y}})=({{n-\delta+y-1 \choose y}}).\frac{y.\delta}{n-\delta}=({{n-\delta+y-1 \choose y-1}}).\delta$
